Covariate Regularized Community Detection in Sparse Graphs

In this paper, we investigate community detection in networks in the presence of node covariates. In many instances, covariates and networks individually only give a partial view of the cluster structure. One needs to jointly infer the full cluster structure by considering both. In statistics, an emerging body of work has been focused on combining information from both the edges in the network and the node covariates to infer community memberships. However, so far the theoretical guarantees have been established in the dense regime, where the network can lead to perfect clustering under a broad parameter regime, and hence the role of covariates is often not clear. In this paper, we examine sparse networks in conjunction with finite dimensional sub-gaussian mixtures as covariates under moderate separation conditions. In this setting each individual source can only cluster a non-vanishing fraction of nodes correctly. We propose a simple optimization framework which provably improves clustering accuracy when the two sources carry partial information about the cluster memberships, and hence perform poorly on their own. Our optimization problem can be solved using scalable convex optimization algorithms. Using a variety of simulated and real data examples, we show that the proposed method outperforms other existing methodology.

==> implementation.tex <==
% Implementation

We use augmented Lagrangian method of multipliers to implement our semidefinite program.
Let $\Phi_i = e_i1_n^T+1_ne_i^T$, then the constraint $X\bfone_n=\bfone_n$ is equivalent to $\innerprod{\Phi_i}{X}=2$.
The problem can be reformulated as
\begin{align*}
\min_X &\quad -\innerprod{A}{X}+\delta(L(X)=b)+\delta(Y\succeq 0)+\delta(0\le Z\le 1/\mmin), \\
s.t. &\quad X=Y, X=Z
\end{align*}
where $\delta(\cdot)$ represents the characteristic function and takes $\infty$ if the condition in the parenthesis is not satisfied. $L(X)_i = \innerprod{\Phi_i}{X}, b_i=2, \forall i \in [n]$, $L(X)_{n+1} = \innerprod{I_n}{X}$, $b_{n+1}=\cl$.

The pseudo code is summarized in Algorithm \ref{alg:admm}. 
In line 5, $\Pi_{S^+}$ computes the projection into the space of semidefinite matrices. To be more explicit, let $X\in \bR^{n\times n}$ be a matrix with eigendecomposition $X=P\Lambda P^T$, $\Lambda =\text{diag}(\lambda_1 \cdots \lambda_n)$. Now we have
\[ \Pi_{S^+}(X) = P\  \text{diag}(\max(0,\lambda_1),\cdots, \max(0,\lambda_n))\  P^T  \]
The projection on line 3 can be calculated in closed form. 
\[ \Pi_L(X)=X-L^*(LL^*)^{-1}(L(X)-b)  \]
where $(LL^*)^{-1}= \begin{bmatrix} \frac{1}{2n}(I_n-\frac{n-2}{n(2n-2)}E) & \frac{1}{n(2-2n)}1_n\\
 \frac{1}{2n(1-n)}1_n^T & \frac{1}{n-1} \end{bmatrix}$.

The stopping criterion is both relative error $\|X^{k+1}-X^k\|/\|X^k\|$ and the infeasibility are less than some tolerance or it achieves a certain number of iterations.
\begin{algorithm}[h!]
\caption{ADMM for solving \sdp{A+\lambda K}}
\label{alg:admm}
\begin{algorithmic}[1]
\REQUIRE Network $A$, node covariate matrix $Y$, tuning parameter $\lambda$, $\rho$.
\STATE Compute kernel matrix $K$ where $K(i,j)=f(\|Y_j-Y_j\|_2^2)$;
\WHILE{not converge}
\STATE $X^{(k+1)}=\Pi_{L}(\frac{1}{2}(Z^k-U^k+Y^k-V^k)+\frac{1}{\rho}(A+\lambda K))$;
\STATE $Z^{(k+1)} = \max(0,X^{k+1}+U^k)$, $Z^{(k+1)} = \min(Z^{(k+1)},1/\mmin)$; 
\STATE $Y^{(k+1)}=\Pi_{S^+}( X^{(k+1)}+V^k )$;
\STATE $U^{(k+1)}=U^{k}+X^{(k+1)}-Z^{(k+1)}$;
\STATE $V^{(k+1)}=V^{k}+X^{(k+1)}-Y^{(k+1)}$;
\ENDWHILE
\STATE Return $X^k$.
\end{algorithmic}
\end{algorithm}

==> mainres-dense.tex <==
\section{Main result}
\label{sec:kernel}
\begin{figure}[t]
\begin{tabular}{c@{\hspace{+3em}}c}
\hspace{-20pt} \includegraphics[width=.5\textwidth]{ve_example_zoom.png} & \includegraphics[width=.45\textwidth]{contour_lightblue.png}\\
(a)&(b)
\end{tabular}
\caption{(a) Example of low dimensional signal plus high dimensional noise. Every row in this matrix is a datapoint in $300$ dimensional space. The zoom in shows the last two columns corresponding to the underlying sparse signal. (b) Error surfaces for sparse graph, \lo covariates and their combination.
}
\label{fig:mc_example}
\end{figure}
It has been well established that sparse and dense graphs have very different theoretical properties in terms of concentration~\citep{le2015sparse}.
Analogously, kernel matrices have different properties in the \hi and \lo settings. To be more specific, when the graph is dense, the adjacency matrix concentrates to its expectation in operator norm~\cite{oliveira2009concentration}. Similarly, in the \hi case, the kernel matrix concentrates elementwise and in Frobenius norm around a suitably defined limit~\citep{el2010information,yan2016robustness}, which is blockwise constant in our subgaussian mixture setting. 
In contrast to the dense case, when graph is sparse, the SDP is not consistent, but can achieve an error rate governed by the within and across cluster probabilities. We present an analogous result for \lo covariates, which establishes that, while SDP with \lo covariates is not consistent, it achieves a small error rate if the cluster centers are further apart.

 %In both cases, we will combine the two sources and see how the outcome improves over that achieved by a single source. We also provide some guideline for the tuning parameters. 
 We first present  the result on dense graph and \hi covariates in subsection \ref{sec:dense_high},
followed by the result for sparse graph and \lo covariates in subsection \ref{sec:sparse_low}. Throughout the remainder of this manuscript, $K$ is the kernel matrix obtained from data, $K(i,j)=f(\|Y_i-Y_j\|_2^2)$, where $f(\cdot)$ is the gaussian kernel function. To be concrete, $
f(x)=\exp(-\eta x)$. 

Let $p_k:=B_{kk}$, $q_k:=\max_{\ell\neq k}B_{k\ell}$, $\pmax = \max_k p_k$ and $\pmin = \min_k p_k$. The distance between clusters $C_k$ and $C_\ell$ is 
\bas{ d_{k\ell}=\|\mu_k-\mu_\ell\|,  \qquad \dmin=\min_{k\ne \ell} d_{k\ell}}
%We will first present our results on dense graphs and high dimensional covariates, followed by sparse graphs and \lo covariates.
\subsection{Dense graph and \hi covariates}
\label{sec:dense_high}
In this section we assume that each covariate consists of low-dimensional information plus high dimensional noise (Equation~\ref{eq:data-model-high}). 
This model allows the distance between the cluster means to remain constant as $n$ grows. Since $K$ concentrates around a blockwise constant matrix, we define the separation for $K$ as: 
\begin{align}
\nu_k:=f(2\sigma_k^2)-\max_{\ell\ne k} f(d^2_{k\ell}+\sigma_k^2+\sigma_\ell^2),
\end{align}
We will use $\nu_k$ as the separation corresponding to the covariate clusters; however it is defined differently in the \hi and \lo cases.
%Note that this definition is different from the one in the \lo case (Equation~\ref{eq:kernel-lodim-sep}). 
%We will start with the main result combining dense graphs and \hi covariates. 
\begin{theorem}[Dense graph plus \hi covariates]
	Define $\nu_k$  as in Equation~\ref{eq:nuk}. For 
	$\gamma' = \min_k \left(\frac{p_k-q_k}{1+\lambda}+\frac{\lambda}{1+\lambda} \nu_k\right)\geq 0$, we have:
	\bas{\frac{\|\hat{X}-X_0\|_F}{\|X_0\|_F}\le \frac{\sqrt{2\alpha^2\cl}}{\gamma'}\left(\frac{1}{1+\sqrt{\lambda}}C_G\sqrt{\frac{r\pmax}{n}}+\frac{\sqrt{\lambda}}{1+\sqrt{\lambda}}C_K\sqrt{\frac{\log n}{\min(d,n)}}\right)}.	%Assume $\cl=o\left( \min\left\{ \frac{n^2\log\dim}{\dim \mmin}, n \right\} \right)$, then \[ \frac{\|\xh-X_0\|_F}{\|X_0\|_F}=o_P(1)\] provided $\gamma=\Omega\left( \max\left\{ \frac{\sqrt{n\pmax}}{\mmin}, \lambda \frac{n}{\mmin}\sqrt{\frac{\log\dim}{\dim \cl}} \right\} \right)$.	
	%If $\gamma'/\sqrt{r\alpha^2}=\Omega\left(\max\left(\sqrt{\frac{r\pmax}{n}},\sqrt{\frac{\log n}{min(n,d)}}\right)\right)$
	%then $\frac{\|\hat{X}-X_0\|_F}{\|X_0\|_F}=o_P(1)$. 
	\label{th:main_g_k}
\end{theorem}
\vspace{-1em}
\textsc{Remark on Orthogonal information content:}
Compared to prior work, the separation condition in Theorems~\ref{th:sparse_low} and~\ref{th:main_g_k} indicates that adding the kernel part allows the SDP to succeed in a larger range of situations. In particular, for each cluster, both of $p_k-q_k$  and $\nu_k$ do not have to be large positive numbers as long as their sum is. We want to point out that, if one of the sources has much stronger signal, it may render the other source useless asymptotically.  However, if $p_k-q_k$ and $\lambda\nu_k$ are of the same order and the separation conditions are satisfied, then one would get a constant times better improvement in the error rate. 

The most interesting scenario arises however, where for some $k$, $p_k-q_k$ is not large enough to satisfy the separation condition on the network, however $\nu_k$ is large and hence putting the two together has a better chance at separating out the $k^{th}$ cluster. That said, it is also possible to get a worse clustering, if one was adverserial and one source was forced to have enough noise to drown the signal from the other. One can, in principle, get around this problem by tuning $\lambda$. The tuning procedure is discussed in detail in Section~\ref{sec:exp}.

The proof of our main result relies on two intermediate results which can be also seen as two special cases of \ref{sdp2}.  Setting $\lambda=0$ we have the following result for weakly assortative block models in the dense case. On the other extreme, by taking $\lambda\rightarrow\infty$ in \ref{sdp2} we provide conditions for the consistency of kernel clustering for \hi covariates. 

\begin{theorem}[Analysis of dense graph]
	Let $\xh$ be the optimal solution of \ref{eq:sdp1}. If  $\min_k (p_k-q_k)>0$,
	then, with probability tending to one, 
	\bas{
	\frac{  \| \xh-X_0\|_F}{\|X_0\|_F} \le \frac{r\alpha}{ \min_k(p_k-q_k)}O_P\left(\sqrt{\frac{\pmax}{n}}\right),
	}
	%where $C_G$ is a positive constant.
	Therefore, 
	\bas{
		\frac{  \| \xh-X_0\|_F}{\|X_0\|_F}=o_P(1)\quad\mbox{if}\quad	\min_k (p_k-q_k)/r\alpha = \Omega(\sqrt{\pmax/n})
	}
	\label{th:dense_graph}
\end{theorem}
\vspace{-1em}
%Furthermore, the result in the dense case implies weak consistency as long as $\frac{\cl (\pmax-\pmin)}{\min_k (p_k-q_k)}=o(n)$, that is, the relative error normalized by the norm of $X_0$ goes to 0 as $n\to \infty$. In the special case when $\pmax=\pmin$, it is able to achieve strong consistency of $\hat{X}$, i.e. $\|\hat{X}-X_0\|_1= 0$ with high probability. 
\textsc{Remark on strong vs. weak consistency:}
A strong consistency result ($\hat{X}=X_0$ w.h.p) for a slightly different SDP was shown in the dense case by \cite{amini2014semidefinite}, under the assumption of equal cluster sizes. In fact, our proof technique can be adapted to recover their result under the same condition. However, under the more general setting of unequal clusters, we can only show weak consistency, i.e. the suitably normalized Frobenius norm of the error converges to zero. 

We now present the result in the \hi covariate setting.

\begin{theorem}[Low noise covariates]
	Let $\hat{X}$ be the solution of the following SDP,
	\begin{equation}\begin{split}
	\qquad \max_X &\quad \innerprod{K}{X},\\
	\qquad s.t. &\ \  X\succeq 0, \ \  0\le X\le 1/m_{\min}, \ \  X\bfone_n= \bfone_n,  \ \  \tr(X)=\cl.
	\label{eq:sdp3}
	\end{split}\tag{SDP-cov}
	\end{equation} 
	where $K$ is the kernel matrix generated from kernel function $f$. Denote \ba{\label{eq:nuk}
		\nu_k:=f(2\sigma_k^2)-\max_{\ell\ne k} f(d^2_{k\ell}+\sigma_k^2+\sigma_\ell^2),
	} 
	and $\alpha:=m_{\max}/\mmin$. If $\min_k\nu_k\geq 0$, for $p=\Omega(\log n)$, there exists a constant $C_K$, such that with probability tending to one, we have:
	\bas{\frac{\|\xhat-X_0\|_F}{\|X_0\|_F}&\leq \frac{C_K }{\min_k\nu_k}\sqrt{\frac{r\alpha^2\log n}{\min(\dim,n)}}
	}
	
	We have $ \frac{\|\xhat-X_0\|_F}{\|X_0\|_F} =o_P(1)$, if
	$
	\min_k\nu_k=
	\Omega\left(\sqrt{\frac{r\alpha^2\log n}{\min(\dim,n)}}\right) .$
	
	%	\Omega\left(\sqrt{\frac{r\alpha^2}{n}}\right) &\mbox{When $d=\Omega(n\log n)$}\\
	%\end{cases}
	%}
	%\bas{
	%\min_k\nu_k=\begin{cases}
	%	\Omega\left(\sqrt{\frac{r\alpha^2\log n}{d}}\right) &\mbox{When  $d=\Omega(r\alpha^2\log n)$ and $O(n\log n)$}\\
	%	\Omega\left(\sqrt{\frac{r\alpha^2}{n}}\right) &\mbox{When $d=\Omega(n\log n)$}\\
	%\end{cases}
	%}
	\begin{comment}
	If $d=o(n)$, then when $\min_k\nu_k=\Omega\left(\sqrt{\frac{r\alpha^2\log n}{d}}\right)$
	If $n\rightarrow \infty$ and $\dim$ grows polynomially with $n$, $\cl=o\left( \frac{n^2\log\dim}{\dim \mmin} \right)$, and $\min_k \nu_k =\Omega\left( \frac{n}{\mmin}\sqrt{\frac{\log \dim}{\dim \cl}}\right)$, then
	\[ \frac{\|\xhat-X_0\|_F}{\|X_0\|_F} =o_P(1).  \]
	\end{comment}
	\label{th:main_kernel}
\end{theorem}

%\textsc{Remark on strong vs. weak consistency.}
%In the current form, we only show weak consistency. 
%This is because of the fact that 
%But when all clusters share the same variance $\sigma_k$, Theorem \ref{th:main_kernel} implies exact recovery of $X_0$. 

Since we use the Gaussian kernel, $\nu_k$ is bounded 
above by one. While the exact value of $\nu_k$ depends on the choice of $\eta$ and the model parameters, lower variance and larger inter-cluster distance will result in larger $\nu_k$. It is important to note that under our model assumption, $d_{k\ell}$  does not increase as dimension $\dim$ goes to infinity.

\input{kernel_low_qs_new}

We now present the tuning procedure, and experimental results.



==> proof_sparse_fro.tex <==
\section{Appendix}
\label{sec:proof_sparse}
\rd
In this section, we present the proof of Lemma~\ref{lem:fro_to_innerprod} and a proof sketch for the sub-gaussian covariates. The analysis for SDP on sparse graph and the combined matrix $A+\lambda K$ are left in supplementary materials due to space contraints.
\bk

\subsection{Proof of Lemma~\ref{lem:fro_to_innerprod}}



\subsection{Analysis of covariates}
The details of the following proof sketch is deferred to the supplementary material. %How much is in the supplementary?\bk
\begin{proof}[Proof sketch of Proposition~\ref{prop:lowdim_kernel}]
Recall that by definition, for $i\in C_k$, $Y_i-\mu_k$ is sub-gaussian random vector with sub-gaussian norm $\psi_k$. Using the following concentration inequality from \cite{hsu2012tail} for sub-gaussian random vectors, we have:
	\begin{align*}
	\mbox{For $i\in C_k$, }P(\|Y_i-\mu_k\|_2^2>\psi_k^2(d+2\sqrt{t\dim}+2t))\le e^{-t}
	\end{align*}	
	%We take  $t = c_k^2 d$ for $c_k\geq 1$. 
	Since $1+2c_k+2c_k^2\leq 5c_k^2$ for $c_k\geq 1$, we get $P(\|Y_i-\mu_k\|^2 \le 5c_k^2\psi_k^2d)\ge 1-\exp(-c_k^2d)$. Let $\Delta_k = \sqrt{5}c_k\psi_k\sqrt{d}$, we can divide the nodes into ``good nodes'' (those close to their population mean) $\cS_k$ and the rest as follows:
	\begin{align}
	\label{eq:csk}
	\cS_k=\{i\in C_k:\|Y_i-\mu_k\|\leq \Delta_k\},\qquad \cS=\cup_{k=1}^\cl \cS_k
	\end{align} 
	Let $m_c^{(k)}=m_k-|\cS_k|$. We want to bound $m_c^{(k)}$ with high probability. Note that $m_c^{(k)}=\sum_{i\in C_k} \bm{1}(\|Y_i-\mu_k\|\geq \Delta_k)$ is a sum of i.i.d random variables. Therefore, using the Hoeffding bound and union bound over all clusters we get:
	\begin{align}
	P\left(m_c \ge \sum_k m_k e^{-c_k^2d}+ \sum_k\sqrt{m_k\log m_k/2}\right)\le \sum_k \frac{1}{m_k}
	\label{eq:chernoff_noutlier}
	\end{align}
	
Now recall $K_I$ is defined as in Eq~\eqref{eq:K_I}.
%define 
%\beq{
%(K_I)_{ij}=\left\{ \begin{matrix} f(2\Delta_k), & \mbox{ if $i,j\in C_k$}\\ \min\{f(d_{k\ell}-\Delta_k-\Delta_\ell),K_{ij}\}, & \mbox{ if $i\in C_k, j\in C_\ell, k\ne \ell$}\end{matrix}\right. 
%\label{eq:K_I}
%}
By construction, all diagonal blocks of $K_I$ are blockwise constant and the off-diagonal blocks are upper bounded by $f(d_{k\ell}-\Delta_k-\Delta_\ell)$. Let $\nu_k = f(2\Delta_k)-\max_{\ell\ne k}f(d_{k\ell}-\Delta_k-\Delta_\ell)$, and $\gamma=\min_k \nu_k$. When $\gamma\geq 0$, by Lemma \ref{lem:fro_to_innerprod},% and Grothendieck's inequality, we have
\ba{
	\label{eq:lowdim_ki}
\|\xh-X_0\|_F^2 \le \frac{2}{\mmin \gamma}\innerprod{K-K_I}{\xh-X_0} \le \frac{2r}{\mmin \gamma} \|K-K_I\|_2
%\le \frac{4K_G}{\mmin^2 \gamma}\llnorm{K-K_I}
}

Now it remains to bound the $\ell_\infty\to\ell_1$ norm of $K-K_I$. Note that if $i\in S_k, j\in S_\ell, k\ne\ell$, then by a simple use of triangle inequality we have $K_{ij}\le f(d_{k\ell}-\Delta_k-\Delta_\ell)$, so $K_{ij}=(K_I)_{ij}$; and if $i,j\in S_k$, then $K_{ij}\ge f(2\Delta_k)$.
\beq{
\bsplt{
&\llnorm{K-K_I} = \max_{x,y\in \{\pm\}^n} \sum_{i,j} x_iy_j\left( K_{ij}-(K_I)_{ij} \right)\\
\le& \max_{x,y\in \{\pm\}^n} \sum_{i,j\in \cS} x_iy_j\left( K_{ij}-(K_I)_{ij} \right)+\max_{x,y\in \{\pm\}^n} \sum_{i \not \in \cS \cup j\not \in \cS} x_iy_j\left( K_{ij}-(K_I)_{ij} \right)\\
%\stackrel{(i)}{\le}& \max_{x,y\in \{\pm\}^n} \sum_{i,j\in \cS} x_iy_j\left( K_{ij}-(K_I)_{ij} \right)+2m_cn\\
\stackrel{(i)}{=}& \max_{x,y\in \{\pm\}^n} \sum_k \sum_{i,j\in \cS_k} x_iy_j\left( K_{ij}-f(2\Delta_k) \right)+2m_cn \le  \sum_k m_k^2(1-f(2\Delta_k))+2m_cn
}
\label{eq:llnorm_kki}
}
where $(i)$ is due to $|K_{ij}-(K_I)_{ij}| \le 1$, and  from the definition of $K_I$. Now Eq~\eqref{eq:lowdim_ki} leads to:
\beq{
\bsplt{
\|\xh-X_0\|_F^2 \le& \frac{4K_G \left( \sum_k m_k^2(1-f(2\Delta_k))+2m_cn \right)}{\mmin^2 \gamma}\\
}
\label{eq:lowdim_sumk}
}

Using some non-trivial algebraic manipulations, which are deferred to the Supplementary, we show that when $\frac{d_{\min}}{\psi_{\max}}>\max(\sqrt{d},180/\sqrt{\dim})$, we have:
	\bas{
		\frac{\|\xh-X_0\|_F^2}{\|X_0\|_F^2} \le& C\alpha^2\max\left( \frac{\psi_{\max}^2d}{\dmin^2} \max\left\{\log\left(\frac{\dmin}{\psi_{\max}\sqrt{d}}\right),r\right\},\cl\sqrt{\frac{\log \mmax}{m_{\max}}}\right)
	}

\end{proof}









==> related.tex <==
\section{Related Work}
\label{sec:related}
For our model, we use the widely known Stochastic Block Model~\cite{holland1983stochastic} as the network model, and a mixture of subgaussian random variables to model the covariates. In a Stochastic Block Model (which we define later), the nodes have fixed latent memberships to $\cl$ clusters which are to be estimated. The nodes within the same cluster are stochastically equivalent, i.e. their probabilistic linkage behavior is identical to each other.

\rd 
~\citet{amini2014semidefinite} define two different classes of block models in terms of separability of blocks. In a strongly assortative blockmodel, linkage probabilities within ``any'' cluster is larger than the ``all'' ${\cl \choose 2}$ linkage probabilities across different clusters. In a weakly assortative blockmodel, the linkage probability within cluster $i$ has to be bigger than $\cl-1$ linkage probabilities between $i$ and $j, j\neq i$. This distinction is important because the weakly assortative class is a superset of strongly assortative models, and most of the analysis are done in the stronger setting. 
\bk
We will first describe related work that incorporates covariates and then focus on existing analysis for individual source of information. 

Some recent works have been focused on incorporating covariates for community detection~\citep{binkiewicz2014covariate, zhang2015community}. In~\cite{binkiewicz2014covariate}, the authors present assortative covariate-assisted spectral clustering (ACASC) where one does Spectral Clustering on the the gram matrix of the covariates plus the regularized graph Laplacian weighted by a tuning parameter. The clusters are estimated using Spectral Clustering on top eigenvectors of the sum. \rd While the method is scalable and is shown to work well in practice, a drawback of the analysis is that in the the covariates are modeled as finite dimensional mixture of bounded random variables, \bl which has a Bayes error in the limit when the distance between the means do not grow with the number of nodes $n$ \rd, whereas in the dense degree regime considered by the authors, the network always leads to perfect clustering. Hence, it is not theoretically clear whether the covariates help improve the accuracy.\bk 
\rd DO THEY ASSUME STRONG ASSORTATIVITY?\bk

%\rd drawback of their method \bk

A joint criterion for community detection (JCDC) with covariates is proposed by~\cite{zhang2015community}, which could be seen as a covariate reweighted Newman-Girvan modularity. This approach enables learning different influence on each covariate. The assumptions include strong assortativity and bounded covariates. In their work, the optimization is carried out in an alternative manner, which is a jointly non-convex problem. Thus although the true maximizer of the JCDC objective is consistent, the algorithm may return a local optima. Notable Bayesian and likelihood-based approaches that include covariates for block models appear in \cite{newman2015structure, yang2013community}.

We complete this section with a brief discussion of related work on theoretical analysis of the clustering performance of each individual view.


\subsection{Related work on analysis of networks}
Typically in asymptotic analysis of networks, one lets the linkage probabilities go to zero in order to allow for sparse graphs. This rate essentially puts different growth conditions on the average degree of the network. We will denote the regime where the average degree grows faster than logarithm of the number of nodes $n$ as the dense case and the regime where the average degree is constant as the sparse case. While most network-based community detection schemes give perfect classification in the limit in the dense case ~\citep{amini2013pseudo,amini2014semidefinite,cai2015robust,chen2014statistical}, in the sparse case one can only achieve near perfect clustering, i.e. a small albeit constant fraction of nodes are misclassified~\citep{guedon2014community,Montanari:2016}.  Most of these works assume strong assortativity, i.e. the smallest within cluster linkage probability is larger than the largest across cluster linkage probability. Recently~\citet{amini2014semidefinite} have provided an SDP which achieves perfect clustering in the dense case for weakly assortative settings. %A model is defined to be weakly assortative when for any cluster $k$ the within cluster probability of linkage is larger than the probability of linking between clusters $k$ and $\ell$, $\forall \ell\neq k$.

%\rd We use a proof technique similar to~\citep{guedon2014community} to establish that our Semidefinite program for sparse weakly assortative block models with different block sizes have good accuracy. \bk

\subsection{Related work on analysis of mixture models}
For covariate clustering, it is common to make distributional assumptions; usually a mixture model with well-separated centers suffices to show consistency. \citet{dasgupta2007probabilistic} use a Gaussian mixture model, and propose a variant of EM algorithm that provably recovers the center of each Gaussian when the minimum distance between clusters is greater than some multiple of the square root of dimension. \citet{awasthi2012improved} work with a projection based algorithm and derive conditions on the separation between the cluster centers for obtaining perfect clustering in the limit. 

Another popular technique is based on SDP relaxations. For example, \citet{peng2007approximating} propose a SDP relaxation for \km type clustering.  In recent work, \citet{mixon2016clustering} show the effectiveness of SDP relaxation with \km clustering for sub-gaussian mixtures, provided the minimum distance between centers is greater than the standard deviation of the sub-gaussian times the  number of clusters $\cl$.

\rd Once we have our analysis we should add the dependence on $\cl$ here.\bk

%Most results focus on the strongly assortative case except~\citet{amini2014semidefinite}, who show that in the dense regime~\ref{eq:sdpold} is consistent even for weakly assortative block models with equal sized clusters. Our result however only establishes weak consistency. The authors also propose a semidefinite relaxation for unequal sized clusters (discussed in Section~\ref{sec:exp}) which is shown to yield reasonable clustering for the population matrix $E[A|Z]$. In Section~\ref{sec:exp}, we show that the constraint set of this SDP requires much heavier computation than~\ref{eq:sdp1}.

\subsection{Our contribution}
Our contribution is two-fold. We show that when the information from the two sources is not aligned, combining them improves the error bound over a broader range of parameters. In addition, we obtain a similar result as in~\citep{guedon2014community} for sparse graphs, which also works for weakly assortative models. Our result on kernel covariate clustering also is comparable to existing separability conditions that depend on the number of clusters $r$, and not the dimension $\dim$ (similar to ~\cite{mixon2016clustering}).
